Third-party Service Dependencies and Centralization Around the World

There is a growing concern about consolidation trends in Internet services, with, for instance, a large fraction of popular websites depending on a handful of third-party service providers. In this paper, we report on a large-scale study of third-party dependencies around the world, using vantage points from 50 countries, from all inhabited continents, and regional top-500 popular websites.This broad perspective shows that dependencies vary widely around the world. We find that between 15% and as much as 80% of websites, across all countries, depend on a DNS, CDN or CA third-party provider.Sites critical dependencies, while lower, are equally spread ranging from 9% and 61% (CDN and DNS in China, respectively).Despite this high variability, our results suggest a highly concentrated market of third-party providers: three third-party providers across all countries serve an average of 91.2% and Google, by itself, serves an average of 72% of the surveyed websites. We explore various factors that may help explain the differences and similarities in degrees of third-party dependency across countries, including economic conditions, Internet development, language, and economic trading partners.

==> sections/dataset.tex <==
\section{Dataset}
\label{sec:Dataset}

The following paragraphs describe the gathered dataset we rely on for our analysis. We downloaded the Alexa Top-100k overall sites and the Alexa Top-500 regional sites for 115 countries in February 2021. We grouped countries in three classes, based on the degree of overlap between their top regional sites and the Top-100k sites overall. We selected 50 countries from each of these three classes, with approximately a third of countries from each class. The set of countries is listed in the appendix. The final set of regional websites for the selected countries includes a total of 25,000 websites with 15,774 unique sites.

From the 15,774 total unique websites, 15,600 use CDNs and 17,001 uses HTTPs. For our CDN analysis, we found a total of 1339871 unique resources and used 877337 unique internal resources. Across all countries we found 68 unique third party CAs, 63 unique third party CDNs and 764 unique third party DNS Providers. 


